Polar codes in quantum information theory

Polar codes are the first capacity achieving and efficiently implementable codes for classical communication. Recently they have also been generalized to communication over classical-quantum and quantum channels. In this work we present our recent results for polar coding in quantum information theory, including applications to classical-quantum multiple access channels, interference channels and compound communication settings, including the first proof of channel coding achieving the Han-Kobayashi rate region of the interference channel without the need of a simultaneous decoder. Moreover we add to the existing framework by extending polar codes to achieve the asymmetric capacity and improving the block error probability for classical-quantum channels. In addition we use polar codes to prove a new achievable rate region for the classical-quantum broadcast channel. We also discuss polar codes for quantum communication over quantum channels and state results towards codes for compound quantum channels in this setting. We conclude by stating a list of interesting open questions to invite further research on the topic.

==> FrontBackmatter/Acronyms.tex <==
%*******************************************************
% Acronyms
%*******************************************************
\automark[section]{chapter}
\renewcommand{\chaptermark}[1]{\markboth{\spacedlowsmallcaps{#1}}{\spacedlowsmallcaps{#1}}}
\renewcommand{\sectionmark}[1]{\markright{\thesection\enspace\spacedlowsmallcaps{#1}}}
%\phantomsection 
\refstepcounter{dummy}
\pdfbookmark[1]{Abk\"{u}rzungsverzeichnis}{abk\"{u}rzungsverzeichnis}
\markboth{\spacedlowsmallcaps{Abk\"{u}rzungsverzeichnis}}{\spacedlowsmallcaps{Abk\"{u}rzungsverzeichnis}}
\chapter*{Abk\"{u}rzungsverzeichnis}

% Insert your acronyms here
\begin{acronym}[UML]
  \acro{DRY}{Don't Repeat Yourself}
  \acro{API}{Application Programming Interface}
  \acro{UML}{Unified Modeling Language}
\end{acronym}

\cleardoublepage


==> FrontBackmatter/Bibliography.tex <==
%********************************************************************
% Bibliography
%*******************************************************
% work-around to have small caps also here in the headline
\manualmark
\markboth{\spacedlowsmallcaps{\bibname}}{\spacedlowsmallcaps{\bibname}} % work-around to have small caps also
%\phantomsection 
\refstepcounter{dummy}
\addtocontents{toc}{\protect\vspace{\beforebibskip}} % to have the bib a bit from the rest in the toc
\addcontentsline{toc}{chapter}{\tocEntry{\bibname}}
\bibliographystyle{plainnat}
\label{app:bibliography} 
\bibliography{IEEEabrv,Bibliography}


==> FrontBackmatter/Listings.tex <==
%*******************************************************
% List of Listings
%*******************************************************      
\automark[section]{chapter}
\renewcommand{\chaptermark}[1]{\markboth{\spacedlowsmallcaps{#1}}{\spacedlowsmallcaps{#1}}}
\renewcommand{\sectionmark}[1]{\markright{\thesection\enspace\spacedlowsmallcaps{#1}}}
%\phantomsection 
\refstepcounter{dummy}
%\addcontentsline{toc}{chapter}{\lstlistlistingname}
\pdfbookmark[1]{\lstlistlistingname}{lol}
\lstlistoflistings

\vspace*{8ex}

\cleardoublepage


==> FrontBackmatter/Tables.tex <==
%*******************************************************
% List of Tables
%*******************************************************
\automark[section]{chapter}
\renewcommand{\chaptermark}[1]{\markboth{\spacedlowsmallcaps{#1}}{\spacedlowsmallcaps{#1}}}
\renewcommand{\sectionmark}[1]{\markright{\thesection\enspace\spacedlowsmallcaps{#1}}}
%\phantomsection 
\refstepcounter{dummy}
%\addcontentsline{toc}{chapter}{\listtablename}
\pdfbookmark[1]{\listtablename}{lot}
\listoftables

\vspace*{8ex}

\cleardoublepage
